Attributed Tree Transducers for Partial Functions

Attributed tree transducers (atts) have been equipped with regular look-around (i.e., a preprocessing via an attributed relabeling) in order to obtain a more robust class of translations. Here we give further evidence of this robustness: we show that if the class of translations realized by nondeterministic atts with regular look-around is restricted to partial functions, then we obtain exactly the class of translations realized by deterministic atts with regular look-around.

==> circular_functional.tex <==
\section{Construction of a Uniformizer for circular $\mathbf{att}$}
In the following, we show that for any  $att$ $A$, regardless of whether it is circular or not,
a $datt^U$ that realizes a uniformizer of $\tau_A$ can be constructed.

Subsequently, let $A=(S,I,\Sigma,\Delta,a_0,R)$ be a  fixed $att$.
We remark that since $A$  may be circular now, the procedure presented in Section~\ref{construction}
for noncircular $atts$ can no longer be applied.
For one, recall that the proof of Lemma~\ref{noncircular eq} relies specifically on the fact that $A$
is noncircular.
Secondly, the circularity of $A$ poses additional challenges for the construction of the
$datt^U$ (see for instance Example~\ref{does not work}).
Particularly, \emph{nonproductive cycles} cause problems.\\ 

\noindent
\textbf{Productive and Nonproductive Cycles.}\quad
Let $s\in \text{dom} (A)$.
Consider trees $t_1,\dots, t_n\in T_\Delta [\text{SI} (s^\#)]$ and let
\[
\tau=(t_1 \Rightarrow_{A,s^\# } t_2 \Rightarrow_{A,s^\# }\cdots \Rightarrow_{A,s^\# } t_n).
\]
We call $\tau$ a translation of $A$ on input $s$ if $t_1=a_0 (1)$.
Since $A$ is circular,
\begin{enumerate}
	\item $\tau$ can contain  a \emph{productive cycle} or
	\item $\tau$ can contain  a \emph{nonproductive cycle}. 
\end{enumerate}
More precisely, 
we say that $\tau$ contains a \emph{productive cycle} if $i<j\leq n$, a node $u$ and a proper descendant $u'$ of $u$
as well as $\ta (\nu) \in \text{SI} (s^\#)$ exist such that
\[
t_i [u]=t_j[u']=\ta (\nu).
\]
On the other hand, if  $i<\iota<j$  and a node $u$ exist such that
\[
t_{i}[u]=t_{j}[u]=\ta (\nu) \quad\text{and}\quad t_{\iota}[u]\neq \ta (\nu),
\]
then we say that  $\tau$ contains a \emph{nonproductive cycle}.

As shown in Example~\ref{does not work}, the fact that 
in the construction of the $datt^U$ $D$ in Section~\ref{construction},
the rules of the underlying $datt$ $A'$ of $D$ are chosen in a basically arbitrary manner
and the fact that in translations of $A$ may contain cycles can cause the procedure in
Section~\ref{construction} to fail if applied to a circular $att$.
Therefore, 


Subsequently, let $A=(S,I,\Sigma,\Delta,a_0,R)$ be a  fixed, functional $att$.
To construct a $datt^U$ $D$ equivalent to $A$,
we must deal with translations of $A$ that are stuck or contain cycles of either type.
Our first step to do so
is to transform $A$ into an equivalent $att^U$ $\hat{A}=(U, A')$
with the following property which we call the \emph{translation-property} (\emph{t-property}).

\subsection{The Translation-Property}
Let $\hat{A}=(U, A')$ be an $att^U$ and let $\hat{A}$ be equivalent to $A$.
Denote by $\hat{a}_0$ the initial attribute of $A'$.
Consider an arbitrary tree
$s\in T_\Sigma$  and let $(s,\breve{s})\in \tau_{U}$. 
In the following, we say that $\hat{A}$ has the \emph{t-property} if for all trees $t$ such that
$
\hat{a}_0 (1)\Rightarrow_{A', \breve{s}^\#}^+ t
$
a tree $g\in T_\Delta$ exist such that  $t \Rightarrow_{A', \breve{s}^\#}^* g$.



Let $s\in\text{dom}(\hat{A})$. Obviously the t-property ensures that
no translation of $A'$ on input  $\breve{s}$  becomes stuck.
As  $A$ is functional and $A$ and $\hat{A}$ are equivalent, the t-property also
guarantees that \emph{no} translation of $A'$ on input $\breve{s}$ 
contains a productive cycle.
To see that the latter holds, assume to the contrary that
$\tau= ( \hat{a}_0 (1)\Rightarrow_{A', \breve{s}^\#} t_1 \Rightarrow_{A', \breve{s}^\#} \cdots \Rightarrow_{A', \breve{s}^\#}  t_n \Rightarrow_{A', \breve{s}^\#} t )$
contains a productive cycle and 
$g\in T_\Delta$ exist so that
$t \Rightarrow_{A', \breve{s}^\#}^* g$.
Then obviously $\hat{A}$ is not functional and hence not equivalent to $A$.

Note that if $s\notin \text{dom}(\hat{A})$ then due to the t-property
no tree $t$ exists such that
$
\hat{a}_0 (1)\Rightarrow_{A', \breve{s}^\#} t.
$

In the following, we construct $\hat{A}=(U, A')$.
The construction idea is similar to the one in Section~\ref{construction}.
Given $\hat{A}$ we show how to deal with translations that contain nonproductive cycles before
constructing $D$.

Before we construct $\hat{A}$, recall the notion of uniform-computation introduced in Section~\ref{construction}.
Furthermore, recall that due to Proposition~\ref{assumption},
we can assume that for $A$ it holds that $R_\#$ is deterministic, i.e., that $R_\#$
contains no distinct rules with the same left-hand side. In particular the following holds.




\begin{construction}{$\mathbf{\hat{A}}$}
	Given the $att$ $A=(S,I,\Sigma,\Delta,a_0, R)$ such that $R_\#$ is deterministic,
	we  construct the $att^U$ $\hat{A}=(U, A')$ with $U=(B,T)$ such that $\hat{A}$ 
	has the t-property and
	is equivalent to $A$.
	
	\textbf{Construction of $\mathbf{A'}$.}\quad
	We define $A'=(S,I,\SigmaU,\Delta, a_0, R^{A'})$.
	The alphabet $\SigmaU$ consists of symbols of the form
	\[
	\sigma^\beta_{\alpha_1,\dots,\alpha_k}
	\text{ where }\sigma\in \Sigma_k,\ k\geq 0,\
	\beta\subseteq I \text{ and }
	\alpha_1,\dots,\alpha_k\subseteq S\times 2^{I} \times \{\top,\bot\}. 
	\]
	The idea is that the look-around $U$
	relabels a tree $s$ over $\Sigma$ into a tree $\breve{s}$ over $\SigmaU$ such that
	the node $v$ is labeled  by $\sigma_{\alpha_1,\dots,\alpha_k}^\beta$ in $\breve{s}^\#$ if and only if 
	\begin{enumerate}
		\item the node $v$ is labeled by $\sigma\in\Sigma_k$ in $s^\#$,
		\item for all $b\in \beta$, a ground tree $t$ exists such that 
		$b(v)\breve{\Rightarrow}_{A,s^\#}^* t$ and
		\item  for all $i\in [k]$, if
		$(a,\beta ,\top)\in \alpha_i$ or $(a,\beta,\bot)\in \alpha_i$, then a ground tree $t$ exists such that $a(v.i)\breve{\Rightarrow}_{A,s^\#}^* t$.
	\end{enumerate}
Note that the reason why unlike the construction
in  Section~\ref{construction},
$\alpha_i$ contains complex tuples of the forms $(a_i,\beta_i ,\top)$ and $(a_i,\beta_i,\bot)$
is because the information stored in these tuples is required to remove nonproductive cycles later.
We will explain these tuples in greater detail when we define the look-around $U$.

The rules of $A'$ are defined analogously as in the construction
in  Section~\ref{construction}.
Let $a\in S$.
For the symbol $\sigma_{\alpha_1,\dots,\alpha_k}^\beta$, we define
$a(\pi) \rightarrow \xi\in R^{A'}_{\sigma_{\alpha_1,\dots,\alpha_k}^\beta}$
if $a(\pi) \rightarrow \xi\in R_\sigma$ and the following holds:
\begin{enumerate}
	\item If $a'(\pi i)$ with $a'\in S$ and $i\in [k]$ occurs in $\xi$ then $\beta\subseteq I$ exists such that
	either
	$(a',\beta ,\top)\in \alpha_i$ or $(a',\beta,\bot)\in \alpha_i$.
	\item If $b(\pi)$  with $b\in I$ occurs in $\xi$ then $b'\in \beta$.
\end{enumerate} 
We proceed analogously for rules in $R^{A'}_{\sigma_{\alpha_1,\dots,\alpha_k}^\beta}$
where an inherited attribute occurs on the left-hand side.
Finally, we define that $R^{A'}_\#=R_\#$.


\textbf{Construction of $\mathbf{B}$.}\quad
We now construct the deterministic bottom-up relabeling~$B=(\mathcal{P},\Sigma,\SigmaB,\mathcal{P},R^B)$.

Informally, $B$ computes how a tree $t$ obtained from a synthesized attribute $a$
processing a tree $s$ in a uniform computation of $A$ looks like, i.e., what inherited attributes occur in $t$ and whether or not
symbols in $\Delta$ occur in $t$.
More precisely, the states in $\mathcal{P}$ are subsets of $S\times (2^{I}\setminus \{\emptyset\} ) \times \{\top,\bot\}$.
The symbols $\bot$ and $\top$ indicate whether or not symbols in $\Delta$ are produced.
In particular, let $P\in \mathcal{P}$ and let $s\in \text{dom}_B (P)$.
Recall that $I_\epsilon$ denotes the set $\{b(\epsilon)\mid b\in I\}$ 
The occurrence of  $(a,\beta,\top)$ with $a\in S$ and $\beta \subseteq I$ in $P$
means that a tree $t\in T_\Delta [I_\epsilon]$ exists
such that 
\begin{itemize}
	\item $a(\epsilon) \breve{\Rightarrow}_{A,s}^* t$ and
	$b(\epsilon)$ occurs in $t$ if and only if $b\in \beta$ and
	\item some symbol in $\Delta$ occurs in $t$.
\end{itemize}
Note that if $\beta=\emptyset$ then this means that $t$ is ground.
Analogously, the occurrence of  $(a,\beta',\bot)$  in $P$ means that a tree $t'\in T_\Delta [I_\epsilon]$ exists
such that 
\begin{itemize}
	\item $a(\epsilon) \breve{\Rightarrow}_{A,s}^* t'$ and $b(\epsilon)$ occurs in $t'$ if and only if $b\in \beta'$ and
	\item no symbol in $\Delta$ occurs in $t'$, i.e., $t'= b(\epsilon)$ and $\beta=\{b\}$ for some $b\in I$. 
\end{itemize}
The set $\SigmaB$ is defined analogously as in  the construction
in  Section~\ref{construction}, i.e., $\SigmaB$ contains symbols of the form 
$\sigma_{P_1,\dots,P_k}$ where $\sigma\in \Sigma_k$, $k\geq 0$, and $P_1,\dots,P_k\in \mathcal{P}$.

Th rules of $B$ are defined as follows.
Let  $\sigma\in \Sigma_k$, $k\geq 0$, and let $P_1,\dots, P_k$ be states of $B$. 
For $i\in [k]$, let $s_i$ be an arbitrary tree in $\text{dom}_B (P_i)$.
Then, we define the rule
\[
\sigma (P_1 (x_1),\dots , P_k (x_k))\rightarrow P(\sigma_{P_1,\dots,P_k} (x_1,\dots x_k)) \in R^B,
\]
where the set $P$ is defined as follows:
\begin{enumerate}
	\item $P$ contains $(a,\beta,\top)$ if and only if
	for $s=\sigma (s_1,\dots, s_k)$, 
	a tree $t\in T_\Delta [I_\epsilon]\setminus I_\epsilon$ exists
	such that 
	$a(\epsilon) \breve{\Rightarrow}_{A ,s}^* t$ and
	$b(\epsilon) \in I_\epsilon$ occurs in $t$ if and only if $b\in \beta$.
	\item $P$ contains $(a,\{b\},\bot)$ if and only if
	$a(\epsilon) \breve{\Rightarrow}_{A ,s}^* b(\epsilon)$
	for $s=\sigma (s_1,\dots, s_k)$.
\end{enumerate}
Since $s$ is a fixed tree, the set $P$ is clearly computable.
As in  the construction in Section~\ref{construction},  $P$ is well-defined, i.e., $P$
is independent of the choice of 
$s_1,\dots,s_k$.
Consider the following.
Let $s\in T_\Sigma$ and let $t,t'\in T_\Delta [SI(s)]$.
Subsequently, we write $t\approx t'$ if 
\begin{enumerate}
	\item[(a)] for all  $\ta (\nu) \in SI(s)$, it holds that
	$\ta (\nu)$ occurs in $t$ if and only if $\ta (\nu)$ occurs in~$t'$ and
	\item[(b)] a symbol in $\Delta$ occurs in $t$ if and only if a symbol in $\Delta$ occurs in $t'$.
\end{enumerate}

The following lemma yields that $P$ is well defined and is shown 
analogously as Lemma~\ref{Order not matter}.

\begin{cclaim}\label{Order not matter circ}
	Let $\sigma \in \Sigma_k$ and let  $P_1,\dots,P_k \in \mathcal{P}$.
	For  $i\in [k]$, let
	$s_i,s_i'\in \text{dom}_B (P_i)$.
	Let $s=\sigma (s_1,\dots,s_k)$ and   $s'=\sigma (s_1',\dots,s_k')$.
	Let $t\in T_\Delta[I_\epsilon]$.
	If $a (\epsilon)\breve{\Rightarrow}_{A,s}^* t$
	then a tree $t'$ exists such that $a (\epsilon)\breve{\Rightarrow}_{A,s'}^* t'$ and $t\approx t'$.
\end{cclaim}

\textbf{Construction of $\mathbf{T}$.}\quad 
In the following, we define $T=(\mathcal{Q},\emptyset,\SigmaB ,\SigmaU,q_0,R^T)$.
The basic idea is the same as in  the construction in Section~\ref{construction}:
$\mathcal{Q}=\{q_0\}\cup 2^I$ such that if for $s\in T_\Sigma$ and $(s,\hat{s})\in \tau_B$, the state $\beta \subseteq I$
arrives at the node $v$ of the tree $\hat{s}^\#$ then the $att$ $A$ can derive
a ground tree from $b(v)$ and the tree~$s^\#$ for all $b\in \beta$.

Symbols in $\SigmaU$ are of the form $\sigma_{\alpha_1,\dots,\alpha_k}^\beta$ 
where $\sigma\in \Sigma_k$, $\beta\subseteq I$ and
$\alpha_1,\dots,\alpha_k\subseteq S\times 2^{I} \times \{\top,\bot\}$ as explained earlier. 


We now define the rules of $T$.
Let $\sigma\in \Sigma_k$ and let $P_1,\dots, P_k$ be states of $B$.
For $i\in [k]$, let $s_i$ be an arbitrary but fixed tree in $\text{dom}_B (P_i)$.
For $q_0$, we define the rule
\[
q_0 (\sigma_{P_1,\dots,P_k} (x_1,\dots, x_k) )\rightarrow  \sigma^\beta_{\alpha_1,\dots,\alpha_k} (\beta_1 (x_1),\dots, \beta_k (x_k))
\]
where $\beta,\beta_1,\dots, \beta_k \subseteq I$ and $\alpha_1,\dots, \alpha_k \subseteq S\times 2^I \times \{\top,\bot\}$
are determined as follows: Let $s=\sigma (s_1,\dots,s_k)$.
\begin{itemize}
	\item We define that $b\in \beta$ if and only if 
	a ground tree~$t$ exists such that
	$
	b (1) \breve{\Rightarrow}_{A,s^\#}^* t.
	$ 
	\item Analogously, for $i\in [k]$, we define that $b\in \beta_i$ if and only if a ground tree $t'$ exists such that
	$
	b (1.i) \breve{\Rightarrow}_{A,s^\#}^* t'
	$.
	\item Let $(a,\beta',\top) \in P_i$. If $\beta' \subseteq \beta_i$ then  $(a,\beta',\top)\in \alpha_i$.
	\item Analogously, let $(a_i,\{b\},\bot) \in P_i$. If  $b\in \beta_i$
	then  $(a,\{b\},\bot)\in \alpha_i$.
\end{itemize}
Note that the definition of this rule is independent of the choice of
$s_1,\dots, s_k$ due to Claim~\ref{Order not matter circ}.
Clearly, for a fixed tree $s$ theses sets are computable.

Recall that for  $\beta \subseteq I$, $\beta_\epsilon$ denotes the set $\{b(\epsilon) \mid b\in \beta\}$.
Consider the state $\beta\subseteq I$.: We define the rule
\[
\beta (\sigma_{P_1,\dots,P_k} (x_1,\dots, x_k) )\rightarrow \sigma^\beta_{\alpha_1,\dots,\alpha_k} (\beta_1 (x_1),\dots, \beta_k (x_k))
\]
where for $i\in [k]$,
$b\in \beta_i$ if and only if for $s=\sigma (s_1,\dots,s_k)$, a tree $t\in T_\Delta [\beta_\epsilon]$
exists such that
$
b (i) \breve{\Rightarrow}_{A,s}^* t.
$ 
Clearly, for a fixed tree $s$, 
all such $b\in I$ are computable.
The sets $\alpha_1,\dots \alpha_k$ are defined the same way as for the $q_0$-rule above.
Note that the construction of these rule of $T'$ is also independent of
the choice of $s_1,\dots,s_k$ due to Claim~\ref{Order not matter circ}.
\end{construction}

\noindent
This concludes the construction of the $att^U$ $\hat{A}$.
Clearly $\hat{A}$ has the t-property.
Before we now show that $A$ and $\hat{A}$ are equivalent, we remark that Observation~\ref{succesful translation}
clearly also holds for circular $atts$. 


\begin{lemma}\label{eq}
	The $att^U$ $\hat{A}=(U,A')$ and the $att$ $A$ are equivalent.
\end{lemma} 

\begin{proof}
	Subsequently, let $s\in T_\Sigma$ and let  $(s,\breve{s}) \in \tau_{U}$.
	First, we show that $\tau_{\hat{A}}\subseteq \tau_A$.
	Let $t\in T_\Delta$ and let $a_0 (1) \Rightarrow_{A',\breve{s}^\#}^* t$.
	Consider $\sigma\in \Sigma_k$ and  $\sigma_{\alpha_1,\dots,\alpha_k}^\beta\in \SigmaU$.
	By construction of the $att$ $A'$, it holds that if  $\rho \in R^{A'}_{\sigma^\beta_{\alpha_1,\dots,\alpha_k} }$ 
	then $\rho \in R_\sigma$.
	This implies   $a_0 (1) \Rightarrow_{A,s^\#}^* t$.
	
	To show that $\tau_{\hat{A}}\supseteq \tau_A$,
	assume that  $a_0 (1) \Rightarrow_{A,{s^\#}}^* t$ where $t$ is ground.
	Due to Observation~\ref{succesful translation} and since $A$ is functional,
	it follows that  $a_0 (1) \breve{\Rightarrow}_{A,{s^\#}}^* t$, i.e., the tree
	$t$ can also be obtained in a uniform computation.
	In particular, let $t_1,\dots,t_n\in T_\Delta [SI (s^\#)]$ such that
	\[
	\tau=(a_0 (1) = t_1  \breve{\Rightarrow}_{A,{s^\#}} t_2  \breve{\Rightarrow}_{A,{s^\#}} \cdots  \breve{\Rightarrow}_{A,{s^\#}} t_n  \breve{\Rightarrow}_{A,{s^\#}} t).
	\]
	Let $v\in V(s^\#)$ such that $s^\# [v]=\sigma$ and $\breve{s}^\# [v]=\sigma^\beta_{\alpha_1,\dots,\alpha_k}$.
	Recall that for a right-hand side $\xi$ of a rule in $R_\sigma$,
	$\xi [\pi\leftarrow v]$ denotes the tree obtained by replacing all occurrences
	of $\pi$ by $v$ (cf. Section~\ref{preliminaries}).
	By construction of $A'$, it is easy to see that the following holds:
	\begin{itemize}
		\item Let $a\in S$.  If the rule $\rho= a(\pi)\rightarrow \xi \in R_\sigma$ is used in $\tau$ at the node $v$,
		i.e., if for some $i \in [n]$, $a(v)$ occurs in $t_i$ and $t_{i+1}$ is obtained from $t_i$ by substituting an
		occurrence of $a(v)$ occurs in $t_i$ by $\xi [\pi\leftarrow v]$,
		then $\rho\in R^{A'}_{\sigma^\beta_{\alpha_1,\dots,\alpha_k}}$.
		\item  Let $b\in I$.  If the rule $\rho= b(\pi j)\rightarrow \xi \in R_\sigma$ with $j\in [k]$ is used in $\tau$ at the node $v$,
		i.e., if for some $i \in [n]$, $b(v.j)$ occurs in $t_i$ and $t_{i+1}$ is obtained from $t_i$ by substituting an
		occurrence of $b(v.j)$ occurs in $t_i$ by $\xi [\pi\leftarrow v]$,
		then $\rho\in R^{A'}_{\sigma^\beta_{\alpha_1,\dots,\alpha_k}}$.
	\end{itemize}
	This implies that $a_0 (1) \breve{\Rightarrow}_{A',{\breve{s}^\#}}^* t$. Thus, our lemma follows. \qed
\end{proof}

To summarize, consider a tree $s\in T_\Sigma$.
Let $\breve{s}$ be the tree such that $(s,\breve{s}) \in \tau_{U}$. 
Recall that due to the t-property, any translation of $A'$ on input $\breve{s}$
cannot contain a productive cycle
if $s\in \text{dom} (\hat{A})$.
Likewise, the t-property yields that any translation of $A'$ on input $\breve{s}$ cannot become
stuck if $s\in \text{dom} (\hat{A})$.
Thus, all that is left is to deal with translations that contain nonproductive cycles. 


\subsubsection{Preprocessing Step.}
Consider the $att^U$ $\hat{A}=(U,A')$.
Before we determinize $\hat{A}$ in order to obtain a $datt^U$ equivalent to $A$,
we require the following preprcessing step for $\hat{A}$:
We modify  $\hat{A}$ such that `\emph{unnecessary}' subcomputations are
omitted. Informally, a  `unnecessary' subcomputation is   a part of a translation of $A'$
in which no output symbols are produced and which hence can be skipped. 
Removing such `useless' subcomputation is a necessary step
in order to avoid translations that contain nonproductive cycles in the future.

Before we go into more detail, consider the following auxiliary lemmas.

\begin{lemma}\label{lemma 1}
	Consider the $att^U$ $\hat{A}=(U,A')$.
	Let $s\in T_\Sigma$ and let $(s,\breve{s}) \in \tau_{U}$.
	Let $v\in V(\breve{s}^\#)$ and $\breve{s}^\# [v]= \sigma^\beta_{\alpha_1,\dots,\alpha_k}$.
	For $i\in [k]$, let $\breve{s}_i= \breve{s}^\#/v.i$. 	Let $a\in S$.
	\begin{enumerate}
		\item[(1)] 	If $(a,\{b\},\bot)\in \alpha_i$, where $b\in I$, then  $a (\epsilon) \Rightarrow_{A' ,\breve{s}_i}^* b (\epsilon)$.
		\item[(2)]  If $(a,\beta',\top)\in \alpha_i$, where $\beta' \subseteq I$, then a tree
		$t\in T_\Delta [I_\epsilon]\setminus I_\epsilon$ exists such that 
		\begin{enumerate}
			\item   $a (\epsilon) \Rightarrow_{A' ,\breve{s}_i}^* t$ and
			\item $b (\epsilon)$, where $b\in I$, occurs in $t$ if and only if $b\in \beta'$.
		\end{enumerate}
	\end{enumerate}
\end{lemma}


\begin{proof}
	Consider the case that $(a,\beta',\top)\in \alpha_i$ for some $\beta' \subseteq I$.
	For $i\in [k]$, denote subsequently by $s_i$ the tree $s^\#/v.i$.

	By construction of $U$, $\breve{s}^\# [v]= \sigma^\beta_{\alpha_1,\dots,\alpha_k}$ with $(a,\beta',\top)\in \alpha_i$
	implies that a tree $t'\in T_\Delta [I_\epsilon]\setminus I_\epsilon$ exists such that
	\begin{enumerate}
		\item[(a)] $a (\epsilon) \breve{\Rightarrow}_{A ,s_i}^* t'$ and
		\item[(b)] $b (\epsilon)$, where $b\in I$, occurs in $t'$ if and only if $b\in \beta'$
	\end{enumerate} 
	due to the definition of the bottom-up relabeling $B$.
	Furthermore, for all $b\in I$ such that $b(\epsilon)$ occurs in $t'$, a ground tree $g$ exists such that
	$b(v.i) \breve{\Rightarrow}_{A ,s^\#}^* g$ due to the definition of the top-down relabeling $T$.
	
	Informally, all rules used by the $att$  $A$ in $a (\epsilon) \breve{\Rightarrow}_{A ,s_i}^* t'$
	are contained in $A'$ as well. 
	More precisely, let $t_1,\dots,t_n\in T_\Delta [SI (s_i)]$ such that 
	\[
	\tau= (a(\epsilon) =t_1 \breve{\Rightarrow}_{A ,s_i} t_2 \breve{\Rightarrow}_{A ,s_i} \cdots \breve{\Rightarrow}_{A ,s_i} t_n =t ).
	\]
	Clearly, this means that 
	\[
	\tau'=  ( a(v.i) =t_1' \breve{\Rightarrow}_{A ,s^\#} t_2' \breve{\Rightarrow}_{A ,s^\#} \cdots \breve{\Rightarrow}_{A ,s^\#} t_n'),
	\]
	where $t_j'= t_j [v\leftarrow \ta (v.i.\nu) \mid v\in V(t_j) \text{ and } t_j[v]= \ta (\nu) \in SI (s_i) ]$ for $j\in [n]$.
	Note that  $b(\epsilon)$, where $b\in I$, occurs in $t_n=t$ if and only if $b(v.i)$ occurs in $t_n'$.
	
	Let $\nu$ be a descendant of the node $v.i$. 
	Let $s^\# [\nu]= \bar{\sigma}$ and $\breve{s}^\# [\nu]=\bar{\sigma}^{\bar{\beta}}_{\bar{\alpha}_1,\dots, \bar{\alpha}_{k'}}$.
	Due to Statement~(b) and
	by construction of $A'$, it follows analogously to Lemma~\ref{eq} that 
	if the rule $\rho\in R_{\sigma'}$ is used in $\tau'$ at the node $\nu$,
	then $\rho\in R^{A'}_{\bar{\sigma}^{\bar{\beta}}_{\bar{\alpha}_1,\dots,\bar{\alpha}_{k'}}}$.
	Obviously, this implies our claim.
	
	The case that $(a, \{b\} ,\bot)\in \alpha_i$ for some $b\in I$  follows analogously.\qed
\end{proof}

\begin{lemma}\label{lemma 2}
	Consider the $att^U$ $\hat{A}=(U,A')$.
	Let $s\in T_\Sigma$ and let $(s,\breve{s}) \in \tau_{U}$.
	Let $v\in V(\breve{s}^\#)$ and let $\breve{s}^\# [v]= \sigma^\beta_{\alpha_1,\dots,\alpha_k}$.
	For $i\in [k]$, let $\breve{s}_i= \breve{s}^\#/v.i$. 
	Let $a\in S$ and $t\in  T_\Delta [I_\epsilon]\setminus I_\epsilon$ such that
	$a (\epsilon) \Rightarrow_{A', \breve{s}_i }^* t$.
	Then some
	$\beta'\subseteq I$ exists such that
	$(a,\beta',\top)\in \alpha_i$.
\end{lemma}

\begin{proof}
	Clearly, 	$a (\epsilon) \Rightarrow_{A', \breve{s}_i }^* t$ where $t\in  T_\Delta [I_\epsilon]\setminus I_\epsilon$
	implies the existence of a tree 
	$t' \in  T_\Delta [I_\epsilon]\setminus I_\epsilon$ such that 	$a (\epsilon) \breve{\Rightarrow}_{A', \breve{s}_i }^* t'$.
	Denote by $\beta'$ the set of all inherited attributes $b$ such that $b(\epsilon)$
	occurs in $t'$.
	
	By construction of~$A'$, $a (\epsilon) \breve{\Rightarrow}_{A',\breve{s}_i}^* t'$ implies that 
	$a (\epsilon) \breve{\Rightarrow}_{A,s_i}^* t'$ holds
	for the $att$ $A$
	and the tree $s_i=s^\#/v.i$.
	
	Obviously, $a (\epsilon) \breve{\Rightarrow}_{A',\breve{s}_i}^* t'$ also implies
	$a (v.i) \breve{\Rightarrow}_{A',\breve{s}_i}^* \tilde{t}$ 
	where $\tilde{t}= [v\leftarrow \ta (v.i.\nu) \mid v\in V(t') \text{ and } t'[v]= \ta (\nu) \in SI (s_i) ]$.
	The definition of the rules of $\hat{A}$  implies that  for all inherited attributes $b$ such that
	$b(v.i)$ occurs in $\tilde{t}$, it holds that a ground tree $g$ exists such that $b (v.i) \breve{\Rightarrow}_{A,s^\#}^* g$.

	By construction of~$U$, this, along with the fact that $a (\epsilon) \breve{\Rightarrow}_{A,s_i}^* t'$,
	means that  $(a,\beta',\top)\in \alpha_i$. \qed
\end{proof}

Let $s\in T_\Sigma$ and let $(s,\breve{s}) \in \tau_U$.
Consider the node $v\in V(\breve{s})$ and let $\breve{s} [v]=\sigma^\beta_{\alpha_1,\dots,\alpha_k}$,
where $\sigma \in \Sigma_k$, $\beta\subseteq I$ and $\alpha_1,\dots,\alpha_k \subseteq S$.
Consider an arbitrary $i\in [k]$.
Assume that all tuples in $\alpha_i$ in which $a\in S$ occurs are of the form
$(a,\{b\},\bot)$ where $b$ is some attribute in $I$; in other words there is no $\beta\subseteq I$ 
such that  $(a,\beta,\top)\in \alpha_i$.
Due to Lemmas~\ref{lemma 1}.(1) and~\ref{lemma 2}, it follows that processing the subtree $\breve{s}_i=\breve{s}/v.i$
with the attribute $a$ 
is unnecessary.
\begin{comment}
	---------NOTIZ-------------------------------
	We need Lemma~\ref{lemma 1} for the following reason.
	Consider $\breve{s}$ and let $v\in V(\breve{s})$.
	If  $\breve{s} [v]=\sigma^\beta_{\alpha_1,\dots,\alpha_k}$  
	and $(a,\beta',\top)\in \alpha_i$ or $(a, \{b\},\bot) \in \alpha_i$  but
	no tree $t\in T_\Delta [I_\epsilon]$ exists such that  $a (\epsilon) \breve{\Rightarrow}_{A' ,\breve{s}/v.i}^* t$
	and $b (\epsilon)$ occurs in $t$ if and only if $b\in \beta'$,
	then the following construction cannot be used.
\end{comment} 
Specifically, when processing $\breve{s}_i$ with the attribute $a$ no output symbols are produced, instead the
translation is continued by some inherited attribute $b$ for which $(a,\{b\},\bot)\in \alpha_i$ holds. 
In other words, instead of processing $\breve{s}_i$ with the attribute $a$, simply
continuing the translation with $b$ is preferable.
Therefore, we will subsequently remove occurrences of $a(\pi i)$ in right-hand sides of rules in 
$R^{A'}_{\sigma^\beta_{\alpha_1,\dots,\alpha_k}}$
skipping the necessity of processing $\breve{s}_i$ with $a$ and continue the translation immediately.

\begin{construction}{the $\mathbf{att^U}$ $\mathbf{\breve{A}=(U, \tilde{A})}$}
We construct the $att^U$ $\breve{A}=(U, \tilde{A})$ from $\hat{A} = (U, A')$ where
$\tilde{A}$ is in essence $A'$ with the property that $\tilde{A}$ skips unnecessary subcomputations.
To construct  $\tilde{A}=(S,I,\SigmaU,\Delta, a_0, R^{\tilde{A}})$
from $A'=(S,I,\SigmaU,\Delta, a_0, R^{A'})$ 
we firstly define $R^{A'}_\# = R^{\tilde{A}}_\#$.

To define the rules for a symbol $\breve{\sigma} = \sigma^\beta_{\alpha_1,\dots,\alpha_k}\in \SigmaU$, we proceed as follows:
Define auxiliary symbols $\theta_1,\dots,\theta_k$ of rank $0$ with which we expand the $att$ $A'$.
For each such auxiliary symbol $\theta_i$ with $i\in [k]$ define the following rules: 
Let $a'\in S$ and $b'\in I$.
If  $(a',\{b'\}, \bot) \in \alpha_i$ and no set 
$\beta'\subseteq I$ exists such that $(a', \beta', \top) \in \alpha_i$,
then define $a' (\pi) \rightarrow b' (\pi) \in R^{A'}_{\theta_i}$.

For each $a\in S$ such that $a(\pi)$ occurs on the left-hand side of some rule in
$R^{A'}_{\breve{\sigma}}$, 
compute for the tree $\breve{s}=\breve{\sigma} (\theta_1,\dots,\theta_k)$
the set 
\[
\mathcal{S}_a=\{ t\in T_\Delta [SI (\breve{s})]  \mid a(\epsilon) \breve{\Rightarrow}_{A' , \breve{s} }^* t \text{ and no tree } t' \text{ exists such that } t  \breve{\Rightarrow}_{A' , \breve{s} }^* t'\}
\]
Note that since $\mathcal{S}_a$ is defined using uniform computations if follows that
$\mathcal{S}_a$
is finite. 
We emphasize that if $t \in \mathcal{S}_a$ then $t$ is obviously a tree in
\[
T_\Delta [I(\epsilon) \cup \{ a' (j)\mid a'\in S,\ j\in [k] \text{ and } \beta'\subseteq I \text{ exists such that }
(a',\beta', \top)\in \alpha_j  \}].
\] 
Given $\mathcal{S}_a$ we now define the rules of $\tilde{A}$ for the symbol $\breve{\sigma}$
where $a(\pi)$ occurs on the left-hand side.
First, recall that as defined in Section~\ref{preliminaries}, $[\pi\leftarrow v]$ denotes the substitution that replaces all occurrences
of $\pi$ by the node $v$.
Furthermore, denote for each $t \in \mathcal{S}_a$  by $\breve{t}$ the tree in
$T_\Delta [\{a'(\pi i) \mid a'\in S, i\in [k]\} \cup \{b'(\pi) \mid b'\in I\} ]$
such that $\breve{t}[\pi\leftarrow \epsilon]= t$. 
For each $t \in \mathcal{S}_a$, we define
$a(\pi) \rightarrow \breve{t} \in R^{\tilde{A}}_{\breve{\sigma}}$.
We remark that by construction it follows that if $a' (\pi j)$ where $a'\in S$ and $j\in [k]$ occurs in 
$\breve{t}$ then some $\beta'\subseteq I$  exists such that 
$(a',\beta', \top)\in \alpha_j$.

For each $b\in I$ and each $j\in [k]$ such that $b(\pi j)$ occurs on the left hand-side of some rule in
$R^{A'}_{\breve{\sigma}}$, we proceed analogously by computing the set
\[
\mathcal{S}_{b,j}=\{ t\in T_\Delta [SI (\breve{s})]  \mid b(j) \breve{\Rightarrow}_{A' , \breve{s} }^* t \text{ and no tree } t' \text{ exists such that } t  \breve{\Rightarrow}_{A' , \breve{s} }^* t'\}.
\]
Then, for each $t \in \mathcal{S}_{b,j}$, we define
$b(\pi j) \rightarrow \breve{t} \in R^{\tilde{A}}_{\breve{\sigma}}$.
This concludes the construction of $\tilde{A}$ and hence the construction of $\breve{A}$.
\end{construction}

\noindent
For the correctness of $\breve{A}$, consider the following.

\begin{lemma}\label{prev}
The $att^U$ $\hat{A} =(U,A')$ and the $att^U$ $\breve{A}=(U, \tilde{A})$ are equivalent.
Furthermore, $\breve{A}$ has the t-property.
\end{lemma}

\begin{proof}
	Let  $s\in T_\Sigma$ and let $(s,\breve{s})\in \tau_{U}$.
	Note that in a uniform computation 
	on input $\breve{s}$ the $att$ $\tilde{A}$ does essentially the same as $A'$
	does; $\tilde{A}$ only skips unnecessary subcomputations.
	Hence, the following claim holds.
	
	\begin{cclaim}\label{circ claim}
		Let $\ta(\nu) \in \text{SI} (\breve{s}^\#)$ and let $ t\in T_\Delta$.
		Then $\ta(\nu) \breve{\Rightarrow}_{\tilde{A}, \breve{s}^\#}^* t$ if and only if 
		$\ta(\nu) \breve{\Rightarrow}_{A', \breve{s}^\#}^* t$.
	\end{cclaim}
	
	Claim~\ref{circ claim} yields that
	$A'$ and $\tilde{A}$ produce the same output tree in a uniform computation on input $\breve{s}$.
	With  Observation~\ref{succesful translation}, it follows that   $\hat{A}$ and  $\breve{A}$ are equivalent.
	
	
	For the second part of our lemma, i.e., to show that  $\breve{A}$ has the t-property
	note that
	if $a_0 (1) {\Rightarrow}_{\tilde{A},\breve{s}^\#}^* \breve{t}$  holds for $\tilde{A}$,
	then  $a_0 (1) {\Rightarrow}_{A',\breve{s}^\#}^* \breve{t}$  holds for $A'$ by construction of $\tilde{A}$.
	Since $A'$ has the t-property, it follows that if $\ta (\nu)$
	occurs in $\breve{t}$, then some tree $t$ exists such that
	$\ta (\nu) \Rightarrow_{A',\breve{s}^\#}^* t$.
	Observation~\ref{succesful translation} and	Claim~\ref{circ claim} yield that $\tilde{A}$ 
	also has the t-property. 
\end{proof}

\noindent
We remark that
since by Lemma~\ref{prev}, $\breve{A}$ is equivalent to $\hat{A}$ and is hence functional,
and since $\breve{A}$ has the t-property, the following holds.
Let $s\in T_\Sigma$ and  $(s,\breve{s})\in \tau_{U}$.
Then no translation of $\tilde{A}$ on input $\breve{s}$  contains a productive cycle.
The argument is the same as for $\hat{A}$. 


In order to subsequently determinize the $att^U$ $\breve{A}=(U, \tilde{A})$, we require the following
auxiliary lemma.
Similar to Lemma~\ref{lemma 1}.(2) for the $att^U$ $\hat{A} =(U,A')$, the following holds for $\breve{A}$.

\begin{lemma}\label{aux aux}
	Consider the $att^U$ $\breve{A}=(U, \tilde{A})$.
	Let $s\in T_\Sigma$ and let $(s,\breve{s}) \in \tau_{U}$.
	Let $v\in V(\breve{s}^\#)$ and $\breve{s}^\# [v]= \sigma^\beta_{\alpha_1,\dots,\alpha_k}$.
	If $(a,\beta',\top)\in \alpha_i$, where $i\in [k]$, then a tree
	$t\in T_\Delta [I_\epsilon]\setminus I_\epsilon$ exists such that  $a (\epsilon) \Rightarrow_{\tilde{A} ,\breve{s}^\#/v.i}^* t$.
\end{lemma}

\begin{proof}
	Consider the $att^U$ $\hat{A} =(U,A')$.
By Lemma~\ref{lemma 1}.(2), it holds that
if $(a,\beta',\top)\in \alpha_i$ then a tree
$t\in T_\Delta [I_\epsilon]\setminus I_\epsilon$ exists such that 
\begin{enumerate}
	\item  $a (\epsilon) \Rightarrow_{A' ,\breve{s}_i}^* t$ and
	\item $b (\epsilon)$, where $b\in I$, occurs in $t$ if and only if $b\in \beta'$.
\end{enumerate}
In particular, by the proof of Lemma~\ref{lemma 1}, $t$ can be obtained in a uniform computation, i.e.,
$a (\epsilon) \breve{\Rightarrow}_{A' ,\breve{s}_i}^* t$
By construction of $\tilde{A}$, it should be clear that $a (\epsilon) \breve{\Rightarrow}_{A' ,\breve{s}_i}^* t$
implies 
$a (\epsilon) \breve{\Rightarrow}_{\tilde{A} ,\breve{s}_i}^* t$.
This yields our lemma.
\end{proof}

\subsubsection{Determinizing Step.}
In the following, we show how to determinize the $att^U$ $\breve{A}=(U, \tilde{A})$ in order to obtain a
$datt^U$ equivalent to $A$. Recall that $\breve{A}$ also has the t-property.


Consider $\tilde{A}=(S,I,\SigmaU,\Delta, a_0, R^{\tilde{A}})$ and a 
symbol $\breve{\sigma} = \sigma^\beta_{\alpha_1,\dots,\alpha_k}\in \SigmaU$.
Recall that by construction of $\tilde{A}$ the following holds:
Let $\xi$ be a right-hand side of some rule in $R^{\tilde{A}}_{\tilde{\sigma}}$.
If $a(\pi j)$ where $a\in S$ and $j\in [k]$ occurs in 
$\xi$ then some $\beta\subseteq I$  exists such that 
$(a,\beta, \top)\in \alpha_j$.
In the following, we call this property the \emph{productive property}.

With the productive property, we subsequently determinize $\breve{A}=(U, \tilde{A})$.
Informally the idea is to remove surplus rules from $\tilde{A}$.
If for $\breve{\sigma}\in \SigmaU$  multiple rules with the same left hand-side occur in 
the rule set
$R^{\tilde{A}}_{\breve{\sigma}}$  then we remove all such rules except one.
In short, the basic idea is similar to the noncircular case discussed in Section~\ref{construction}.
However unlike the noncircular case where the rules which are removed and the rule that is kept are 
determined  in a basically arbitrary manner, we need to be more specific
in order to avoid cycles.

\begin{construction}{the $\mathbf{datt^U}$  $\mathbf{D=(U, D')}$}
Consider the $att^U$ $\breve{A}=(U, \tilde{A})$ where  $\tilde{A}=(S,I,\SigmaU,\Delta, a_0, R^{\tilde{A}})$.
Subsequently, we construct an equivalent  $datt^U$  $D=(U, D')$
where $D'= (S,I,\SigmaU,\Delta, a_0, R^{D'})$ where $R^{D'}$ is constructed as follows.

Let $a\in S$ and $\breve{\sigma} \in \SigmaU$.
The rule for $a$ and $\breve{\sigma}$ for the set $R^{D'}_{\breve{\sigma}}$ is determined with the following
procedure:
Denote by $R^{\tilde{A}}_{\breve{\sigma},a}$ the set of all rules in $R^{\tilde{A}}_{\breve{\sigma}}$ in which
$a(\pi)$ occurs on the left hand-side. Define a total order on the set $R^{\tilde{A}}_{\breve{\sigma},a}$.
\begin{enumerate}
	\item Let $\rho$ be the first rule in the given order on $R^{\tilde{A}}_{\breve{\sigma},a}$ such that a symbol in $\Delta$ occurs on the right-hand side of $\rho$. 
	\item If such a rule does not exist then 
	let $\rho$ be the first rule in the given order on $R^{\tilde{A}}_{\breve{\sigma},a}$ such that
	$\rho$ is of the form $a(\pi)\rightarrow a' (\pi j)$ where $a'\in S$ and $j\in [k]$.
	\item In the case that no rules of the  forms specified above exist, i,e.,
	if the rule $\rho_j$ is of the form $a(\pi) \rightarrow b (\pi)$ where $b\in I$ for all $j\in [k]$,
	then let $\rho$ be the first rule in the given order on $R^{\tilde{A}}_{\breve{\sigma},a}$.
\end{enumerate}
Then we define $\rho \in R^{D'}_{\breve{\sigma}}$.

The rule in $R^{D'}_{\breve{\sigma}}$ for an inherited attribute $b\in I$ and $\breve{\sigma} \in \SigmaU$ is obtained analogously.
\end{construction}

Choosing rules of $R^{'}$ with this procedure has the following purpose:
$D'$ produces output symbols whenever possible.
Informally, if a rule produces
output symbols then that rule cannot be part of a nonproductive cycle.
Hence, we can use this property to deal with nonproductive cycles.

In particular with the t-property and the productive property of $\breve{A}$,
we subsequently show that neither productive nor nonproductive cycles occur 
in translations of $D'$. To do so, we require the following  auxiliary lemma.

\begin{lemma}\label{appendix aux}
	Consider the  $datt^U$ $D=(U, D')$ with $D'= (S,I,\SigmaU,\Delta, a_0, R^{D'})$.
	An equivalent  $datt^U$ $\hat{D} =(U,\hat{D}')$ with 
	$\hat{D'} = (S,\hat{I},\SigmaU,\Delta, a_0, R^{\hat{D}'})$ can be constructed such that 
	the following holds:
	Let $s\in T_\Sigma$ and let $(s,\breve{s})\in \tau_{U}$.
	Then no $b\in \hat{I}$ and no attributes $\ta_1,\dots,\ta_n\in S\cup \hat{I}$ with $n>0$ exist such that 	
	$b(1) \Rightarrow_{\hat{D}', \breve{s}^\#} \ta_1 (1) \Rightarrow_{\hat{D}', \breve{s}^\#} \ta_2 (1) \Rightarrow_{\hat{D}', \breve{s}^\#} \cdots  \Rightarrow_{\hat{D}', \breve{s}^\#} \ta_n (1)\Rightarrow_{\hat{D}', \breve{s}^\#} b(1)$.
\end{lemma}

\begin{proof}	
	To construct $\hat{D'}$,
	we first transform $D'$ into the auxiliary $datt$ $D''=(S,\hat{I},\SigmaU,\Delta, a_0, R^{D''} )$ where
	$\hat{I}=\{b_{\sigma} \mid b\in I,\sigma\in \SigmaU \}$.
	Informally, each inherited attribute `knows' from which symbol in $\SigmaU$ it originated from.
	
	To define the rules of $D''$, first consider the following definition.
	Let $\sigma\in \SigmaU$ and 
	let $\xi \in T_\Delta [\{a(\pi i) \mid a\in S, i\in [k]\} \cup \{b(\pi) \mid b\in I\} ]$.
	Subsequently, we denote by $\langle \xi\rangle_{\sigma}$
	the tree obtained from $\xi$
	by substituting all occurrences of labels of the form 
	$b(\epsilon)$ in $\xi$, where $b\in I$,  by $b_{\sigma} (\epsilon)$.
	For instance, if $\xi =f( a (\pi 1), b_1 (\pi), b_2 (\pi) )$ where $a\in S$ and $b_1,b_2 \in I$ then 
	$\langle \xi\rangle_{\sigma}=  f( a (\pi 1), {b_1}_{\sigma} (\pi),  {b_2}_{\sigma} (\pi))$.
	
	The rules of $D''$ are defined as follows:
	Let $\sigma\in \SigmaU$ be of rank $k\geq 0$. Let $a\in S$.
	If $a(\pi) \rightarrow \xi \in R^{D'}_{\sigma}$ then $a(\pi) \rightarrow \langle \xi\rangle_{\sigma} \in R^{D''}_{\sigma}$.
	
	Let $b\in I$, $j\in [k]$,  and let $\sigma'$ be an arbitrary symbol in $\in \SigmaU$.
	If  $b(\pi j) \rightarrow \xi \in R^{D'}_{\sigma}$ then
	$b_{\sigma'} (\pi j) \rightarrow   \langle \xi\rangle_{\sigma} \in R^{D''}_{\sigma}$.
	
	Finally, we define that for each $b\in I$ and each $\sigma \in \SigmaU$, if 
	$b (\pi 1) \rightarrow  \xi \in R^{D'}_{\#}$ then
	$b_{\sigma} (\pi 1) \rightarrow  \xi \in R^{D''}_{\#}$. Note that if $b (\pi 1) \rightarrow  \xi \in R^{D'}_{\#}$
	then no inherited attributes occur in $\xi$. 
	
	It should be clear that $D''$ and $D'$ are equivalent.
	Given the rule sets $R^{D''}_{\#}$ and $R^{D''}_{\sigma}$ of $D''$, we can easily compute 
	the set $\mathcal{I}$ of all $b_\sigma\in \hat{I}$ for which some
	tree
	of the form $\breve{s} = \sigma (s_1,\dots, s_k) \in T_{\SigmaU}$
	and $\ta_1,\dots,\ta_n\in S\cup \hat{I}$ with $n>0$ 
	exist such that
	\begin{equation}\label{aux eq}
		b_\sigma(1) \Rightarrow_{D'', \breve{s}^\#} \ta_1 (1) \Rightarrow_{D'', \breve{s}^\#} \ta_2 (1) \Rightarrow_{D'', \breve{s}^\#} \cdots  \Rightarrow_{D'', \breve{s}^\#} \ta_n (1)\Rightarrow_{D'', \breve{s}^\#} b_\sigma(1)
	\end{equation}
	since $D''$ is deterministic.
	The $datt$	$\hat{D}' = (S,\hat{I},\SigmaU,\Delta, a_0, R^{\hat{D}'})$ is obtained from $D''$ by removing all
	rules where an attribute in $\mathcal{I}$ occurs on the left-hand side from  $R^{D''}_{\#}$.
	
	To see that $D''$ and $\hat{D}'$ (and hence to see that $D'$ and $\hat{D}'$) are equivalent,
	consider an arbitrary $b_\sigma \in \mathcal{I}$, a tree $\breve{s} = \sigma (s_1,\dots, s_k) \in T_{\SigmaU}$ and
	a tree $t\in T_\Delta [S\hat{I} (\breve{s}^\#)]$ such that
	$a_0 (1) \Rightarrow_{D'', \breve{s}^\#}^* t$ and $b_\sigma (1)$ occurs in $t$.
	Due to~(\ref{aux eq}) and since $D''$ is deterministic, it follows that $\breve{s}\notin \text{dom} (D'')$. Thus, removing 
	all
	rules where an attribute in $\mathcal{I}$ occurs on the left-hand side from  $R^{D''}_{\#}$
	does not alter the translation realized by~$D''$.\qed
\end{proof}

Due to Lemma~\ref{appendix aux}, we subsequently assume that the following holds for the $datt^U$ $D=(U, D')$:
If $s\in T_\Sigma$ and  $(s,\breve{s})\in \tau_{U}$,
then no $b\in I$ and no attributes $\ta_1,\dots,\ta_n\in S\cup I$ with $n>0$ exist such that 	
\[
b(1) \Rightarrow_{D', \breve{s}^\#} \ta_1 (1) \Rightarrow_{D', \breve{s}^\#} \ta_2 (1) \Rightarrow_{D', \breve{s}^\#} \cdots  \Rightarrow_{D', \breve{s}^\#} \ta_n (1)\Rightarrow_{D', \breve{s}^\#} b(1).
\]
We now prove the following.

\begin{lemma}\label{no cycle}
	Consider $D=(U, D')$.
	Let  $s\in T_\Sigma$ and let $(s,\breve{s})\in \tau_{U}$.
	Neither productive nor nonproductive cycles occur in translations of $D'$ on input $\breve{s}$.
\end{lemma}

\begin{proof}
	First, we show that no productive cycles occur in translations of $D'$ on input $\breve{s}$.
	Let 
	\begin{equation}\label{eq 1}
	a_0 (1) =t_1 \Rightarrow_{D', \breve{s}^\#} \dots \Rightarrow_{D', \breve{s}^\#} t_n,
		\end{equation}
	where $n>1$, be an arbitrary translation of $D'$ on input $\breve{s}$.
	Consider the $att^U$ $\breve{A}=(U, \tilde{A})$ where  $\tilde{A}=(S,I,\SigmaU,\Delta, a_0, R^{\tilde{A}})$.
	By construction of $D$, it follows that
	\begin{equation}\label{eq 2}
		a_0 (1) =t_1\Rightarrow_{\tilde{A}, \breve{s}^\#}  \dots \Rightarrow_{\tilde{A}, \breve{s}^\#} t_n.
	\end{equation}
	Recall that $\hat{A}$ has the t-property.
	Therefore and since $n>1$, it follows that a ground tree $t$ exists such that $t_n\Rightarrow_{\tilde{A}, \breve{s}^\#}^* t$.
	Since $\breve{A}$ is functional, we thus conclude that~(\ref{eq 2})
	cannot contain a productive cycle. 
	This implies that~(\ref{eq 1}) cannot contain a productive cycle and hence our claim.
	
	Now assume that a nonproductive cycle occurs in some translation of $D'$ on input~$\breve{s}$.
	Obviously, this means that $\ta (\nu)\in \text{SI} (\breve{s}^\#)$ exist such that
	$\ta (\nu) \Rightarrow_{D', \breve{s}^\#}^+ \ta (\nu)$.
	Obviously,  $\ta (\nu) \Rightarrow_{D', \breve{s}^\#}^+ \ta (\nu)$ involves a transition of the form $b(v)  \Rightarrow_{D', \breve{s}^\#} a(v)$,
	where $v\in V(\breve{s}^\#)$,  $a\in S$ and $b\in I$.
	In other words, it holds that
	\[
	\ta (\nu) \Rightarrow_{D', \breve{s}^\#} \cdots  \Rightarrow_{D', \breve{s}^\#}   b(v)  \Rightarrow_{D', \breve{s}^\#} a(v)  \Rightarrow_{D', \breve{s}^\#} \cdots  \Rightarrow_{D', \breve{s}^\#} \ta (\nu).
	\]
	This implies
	\begin{equation}\label{eq 3}
		a(v)\Rightarrow_{D', \breve{s}^\#} \cdots  \Rightarrow_{D', \breve{s}^\#} \ta (\nu) \Rightarrow_{D', \breve{s}^\#} \dots \Rightarrow_{D', \breve{s}^\#} b(v)  \Rightarrow_{D', \breve{s}^\#} a(v).
	\end{equation}
    Let $t\in T_\Delta [I_\epsilon]$.
	In the following, we show  that 
	if $a(\epsilon) \Rightarrow_{D', \breve{s}^\#/v}^*t$ then 
	a symbol in $\Delta$ occur in $t$. This contradicts
	$a(v) \Rightarrow_{D', \breve{s}^\#}^* b(v)$ 
	and thus (\ref{eq 3}). This in turn means that in all translation of $D'$ on input~$\breve{s}$,
	no nonproductive cycle occurs.
	
	W.l.o.g. assume that $v$ is the first child node of its parent node. 
	Furthermore, assume that the parent node of $v$ be labeled by 
	$\breve{\sigma}=\sigma^\beta_{\alpha_1,\dots,\alpha_k}$ in 
	$\breve{s}^\#$. The case that the parent node of $v$ is the root marker is examined later.
	Due to (\ref{eq 3}), it follows 
	that $b(\pi 1) \rightarrow a (\pi 1) \in R^{D'}_{\breve{\sigma}}$.
	Due to the productive property of $\breve{A}$ and by construction of $D$,
	this means that $(a,\beta_1,\top)\in \alpha_1$ for some $\beta_1\subseteq I$.
	
	We subsequently prove the following claim by structural induction which implies that
	if $a(\epsilon) \Rightarrow_{D', \breve{s}^\#/v}^*t$ then 
	a symbol in $\Delta$ occur in $t$.
	
	\begin{cclaim}\label{no cycle claim}
		Let $v \in V(\breve{s}^\#)$ and $\bar{v}$ be the parent node of $v$, Let $\bar{v}$ be labeled by 
		$\sigma^\beta_{\alpha_1,\dots,\alpha_k}$ in $\breve{s}^\#$ and let $v$ be the $i$-th child of $\bar{v}$.
		Let $(a,\beta',\top) \in \alpha_i$.
		If $t\in T_\Delta [I_\epsilon]$ exists such that
		$a(\epsilon) \Rightarrow_{D', \breve{s}^\#/v}^*t$
		then  a symbol in $\Delta$ occur in $t$.
	\end{cclaim}
	
	\begin{proof}
		Subsequently, denote by $\bar{s}$ the tree $\breve{s}^\#/v$.
		
		Assume that  $v$ is a leaf i.e., that $\bar{s}=e$ is  a symbol of rank $0$.
		Consider Lemma~\ref{aux aux}.	
		Since $\bar{v}$ is labeled by 
		$\sigma^\beta_{\alpha_1,\dots,\alpha_k}$ and $(a,\beta',\top) \in \alpha_i$,
		Lemma~\ref{aux aux} yields that
		$R^{\tilde{A}}_e$
		contains a rule in which $a(\pi)$ occurs on the left-hand side and
		some symbol in $\Delta$ occurs on the right-hand side.
		By construction of $D$, this means that $R^{D'}_e$ contains such a rule as well
		which yields our claim.
		
		Now assume that $v$ is not a leaf.
		Let $v$ be labeled by $\breve{\sigma}'= \sigma'^{\beta'}_{\alpha_1',\dots, \alpha'_{k'}}$ in 
		$\breve{s}^\#$,  where $k'>0$.
		Since $\bar{v}$ is labeled by 
		$\sigma^\beta_{\alpha_1,\dots,\alpha_k}$ and $(a,\beta',\top) \in \alpha_i$, Lemma~\ref{aux aux} yields that
		the rule set $R^{\tilde{A}}_{\breve{\sigma}'}$ cannot only contain rules of the form $a(\pi)\rightarrow b'(\pi)$ where $b'\in I$
		for the synthesized attribute $a$.
		In other words, at least one  of the following statements holds
		\begin{enumerate}
			\item[(a)] $a(\pi) \rightarrow \xi \in  R^{\tilde{A}}_{\breve{\sigma}'}$ such that some symbol in $\Delta$ occurs in $\xi$ or 
			\item[(b)] $a(\pi) \rightarrow a' (\pi j) \in R^{\tilde{A}}_{\breve{\sigma}'}$ where $a'\in S$ and $j\in [k']$.
		\end{enumerate}
		Clearly if $(a)$ holds then by construction of $D$, the rule set   $R^{D'}_{\breve{\sigma}'}$ contains a rule
		of the form  $a(\pi) \rightarrow \xi'$ such that some symbol in $\Delta$ occurs in $\xi$, 
		which yields our claim.
		
		Now assume that $(a)$ does not hold and that only $(b)$ holds.
		Then by construction of $D$, the rule set $R^{D'}_{\breve{\sigma}'}$ must contain
		the rule of the form $a(\pi) \rightarrow a' (\pi j)$  where $a'\in S$ and $j\in [k']$.
		Note that due to the productive property of $\breve{A}$ and  by construction of $D$,  $a(\pi) \rightarrow a' (\pi j) \in R^{D'}_{\breve{\sigma}'}$ implies that
		some $\beta_j\in I$ exists such that
		$(a',\beta_j,\top) \in \alpha_j'$. 
		Therefore, 
		by structural induction, it follows that 
		if a tree $\bar{t}\in T_\Delta [I_\epsilon]$
		exists such that
		$a' (\epsilon) \Rightarrow_{D', \bar{s}/j}^*\bar {t}$ then 
		some symbol in $\Delta$ occurs in
		$\bar{t}$.
		Together with the fact that  $R^{D'}_{\breve{\sigma}'}$ contains
		the rule  $a(\pi) \rightarrow a' (\pi j)$ this yields our claim.\qed
	\end{proof}

	In the following, we consider the case that the parent node of $v$ is the root marker, i.e., $v=1$ and thus
	\begin{equation}\label{eq 4}
		a(1) \Rightarrow_{D', \breve{s}^\#} \dots \Rightarrow_{D', \breve{s}^\#} b(1)  \Rightarrow_{D',\breve{s}^\#} a(1).
	\end{equation}
	Let $\breve{s}^\# [1]=\sigma^\beta_{\alpha_1,\dots\alpha_k}$. Obviously,  (\ref{eq 4}) implies that trees $t_1,\dots,t_n$ exist such that
	\begin{equation}\label{eq 5}
		b(1) \Rightarrow_{D', \breve{s}^\#} t_1 \Rightarrow_{D', \breve{s}^\#} \dots \Rightarrow_{D',\breve{s}^\#} 
		t_n\Rightarrow_{D', \breve{s}^\#}  b(1).
	\end{equation}
	Recall that due to our previous assumption for the $datt^U$ $D=(U, D')$, some  $i\in [k]$ exists such that
	 $t_i\notin \in \{\ta (1)\mid \ta\in S\cup I\}$.
	W.l.o.g. let $i$ be the first indice such that $t_i\notin \{\ta (1)\mid \ta\in S\cup I\}$.
	Obviously this means that $t_i$ is of the form $t_i=  \tilde{a} (1.j)$ where $\tilde{a}\in S$ and $j\in [k]$.
	Clearly, $t_i$ implies that
	$R^{D'}_{\sigma^\beta_{\alpha_1,\dots,\alpha_k}}$ contains some rule where
	$\tilde{a} (\pi j)$ occurs on the right-hand side. By construction of $D'$, this implies that
	some $\beta_j\subseteq I$ must exist such that $(\tilde{a},\beta_j,\top) \in \alpha_j$.
	Due to Claim~\ref{no cycle claim}, this implies that if $t\in T_\Delta [I_\epsilon]$ exists such that
	$\tilde{a}(\epsilon) \Rightarrow_{D', \breve{s}^\#/1.1 }^*t$ then 
	symbols in $\Delta$ occur in
	$t$ contradicting~(\ref{eq 5}).  \qed
\end{proof}


\begin{lemma}
	The $att^U$ $D=(U, D')$ and $A$ are equivalent.
\end{lemma}
\begin{proof}
	By Lemmas~\ref{eq} and~\ref{prev}, it is sufficient to show that
	$D$ and $\breve{A}=(U, \tilde{A})$ where  $\tilde{A}=(S,I,\SigmaU,\Delta, a_0, R^{\tilde{A}})$ are equivalent.
	By construction of $D$, obviously $\tau_{D}\subseteq \tau_{\breve{A}}$.
	
	For the converse statement, 
	note that by construction of $D$ the following holds:
	The rule set of $D'$
	for the symbol $\sigma \in \SigmaU$
	contains a rule with left hand-side $\zeta$ if and only if the rule set of $A'$
	for the symbol $\sigma$
	contains a rule with left hand-side $\zeta$ $(*)$.
	
	Let $s\in T_\Sigma$ and $(s,\breve{s})\in \tau_{U}$.
	If $s\notin \text{dom} (\breve{A})$ then no ground tree $t$ exists such that $a_0 (\epsilon) \Rightarrow_{D', \breve{s}^\#}^* t$
	since $\tau_{D}\subseteq \tau_{\breve{A}}$.
	Assume that $s\in \text{dom} (\breve{A})$ and let	 
	$
	a_0 (1) =t_1 \Rightarrow_{D', \breve{s}^\#} \dots \Rightarrow_{D', \breve{s}^\#} t_n
	$
	where $n\geq 1$. Assume $t_n$ is not  ground. By construction of $D$, this implies
	$
	a_0 (1) =t_1 \Rightarrow_{\tilde{A}, \breve{s}^\#} \dots \Rightarrow_{\tilde{A}, \breve{s}^\#} t_n.
	$
	Due to the t-property of $\breve{A}$ and $(*)$, it follows that
	a tree $t_{n+1}$ exists such that  $t_n \Rightarrow_{D', \breve{s}^\#} t_{n+1}$.
	Since by Lemma~\ref{no cycle},
	translations of $D'$ on input $\breve{s}$ do not contain cycles, it follows that sooner or later
	we arrive at a ground tree.
	This yields our claim.
\end{proof}

==> old_introduction.tex <==
\section{Introduction}


\begin{center}
	\begin{tabular}{ l|| c }
		Class of Transduction & \ \ functional = deterministic?\\\hline
		One-Way Transduction\ & no   \\
		Two-Way Transduction\ & yes     \\
		Top-Down Tree Transduction\ \ & no   \\ 
		Bottom-Up Tree Transduction\ \ & no    \\ 
		Macro Tree Transduction\ & yes  
	\end{tabular}
\end{center}
The equality of transductions realized by 
deterministic and functional two-way transducers is shown in \cite{Engelfriet1999MSODS}, see also~\cite{DBLP:conf/lata/Souza13}.
For macro tree transducers the same result is shown in~\cite{DBLP:journals/acta/EngelfrietIM21}.
As for the inequality of transductions realized by functional and deterministic
one-way transducers, consider the translation which on input 
$s$ outputs $s$ if the first and the last character  of the input string is $e$; otherwise~$e'$ is outputted.
This example also implies the same result for top-down and bottom-up tree transducers.


class of translations realizable by functional top-down tree transducers with look-ahead also
includes class of functional bottom-up tree transductions


MSO tree-to-tree transducer unknown


look-around more natural extension of att

